Quasi-Probabilistic Readout Correction of Mid-Circuit Measurements for Adaptive Feedback via Measurement Randomized Compiling

Quantum measurements are a fundamental component of quantum computing. However, on modern-day quantum computers, measurements can be more error prone than quantum gates, and are susceptible to non-unital errors as well as non-local correlations due to measurement crosstalk. While readout errors can be mitigated in post-processing, it is inefficient in the number of qubits due to a combinatorially-large number of possible states that need to be characterized. In this work, we show that measurement errors can be tailored into a simple stochastic error model using randomized compiling, enabling the efficient mitigation of readout errors via quasi-probability distributions reconstructed from the measurement of a single preparation state in an exponentially large confusion matrix. We demonstrate the scalability and power of this approach by correcting readout errors without matrix inversion on a large number of different preparation states applied to a register of eight superconducting transmon qubits. Moreover, we show that this method can be extended to mid-circuit measurements used for active feedback via quasi-probabilistic error cancellation, and demonstrate the correction of measurement errors on an ancilla qubit used to detect and actively correct bit-flip errors on an entangled memory qubit. Our approach enables the correction of readout errors on large numbers of qubits, and offers a strategy for correcting readout errors in adaptive circuits in which the results of mid-circuit measurements are used to perform conditional operations on non-local qubits in real time.

==> tables/qubit_readout_properties.tex <==
\begin{table*}[!htbp]
\renewcommand{\arraystretch}{1.5}

\centering
\resizebox{1.75\columnwidth}{!}{
\begin{tabular}{l | r r r r r r r r }
    \hline
    \hline
    {} & Q0 & Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 \\
    \hline
    $T_1$ ($\mu$s) & 74.0(6.8) & 129.0(3.5) & 154.0(3.4) & 49.7(1.1) & 134.0(3.7) & 82.0(2.5) & 53.5(1.2) & 19.9(0.2) \\
    $T_{2E}$ ($\mu$s) & 36.0(1.9) & 39.0(2.6) & 77.0(3.2) & 40.0(1.9) & 50.0(2.2) & 47.0(2.2) & 40.0(1.9) & 28.0(2.1) \\
    RB iso. ($10^{-3}$) & 1.1(1) & 0.75(4) & 1.7(3) & 0.87(8) & 0.65(3) & 0.56(3) & 2.5(3) & 4.6(5) \\
    RB sim. ($10^{-3}$) & 5.3(9) & 2.7(2) & 2.9(3) & 3.1(2) & 7.0(5) & 5.7(3) & 3.4(3) & 7.6(9) \\
    CB sim. ($10^{-2}$) & & & & 4.5(2) & & & & \\
    \hline
    \hline
\end{tabular}}
\caption{Qubit characterization. Qubit coherence times ($T_1$ and $T_2E$) are listed above. The process infidelities for isolated and simultaneous single-qubit randomized benchmarking (RB) are listed as well. The average process infidelity of a cycle of simultaneous Paulis is measured using cycle benchmarking (CB).}
\label{tab:qubit_properties}

\bigskip

\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{l | r r r r r r r r }
    \hline
    \hline
    {} & Q0 & Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 \\
    \hline
    $P(0 | 0)$ & 0.989(2) & 0.981(2) & 0.968(3) & 0.975(2) & 0.967(3) & 0.988(3) & 0.978(3) & 0.985(3) \\
    $P(1 | 1)$ & 0.509(8) & 0.918(4) & 0.941(4) & 0.476(6) & 0.893(5) & 0.617(6) & 0.936(5) & 0.909(5) \\
    \hline
    \hline
\end{tabular}}
\caption{Individual readout fidelities for all qubits without excited state promotion. $P(0|0)$ is the probability of measuring 0 when the qubit is prepared in $\ket{0}$, and $P(1|1)$ is the probability of measuring 1 when the qubit is prepared in $\ket{1}$. $P(1|1)$ is abnormally low for some qubits because the readout amplitudes have been optimized for use with ESP.}
\label{tab:isolated_readout_fidelities}

\bigskip

\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{l | r r r r r r r r }
    \hline
    \hline
    {} & Q0 & Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 \\
    \hline
    $P(0 | 0)$ & 0.989(2) & 0.982(3) & 0.966(3) & 0.976(3) & 0.966(2) & 0.987(2) & 0.980(3) & 0.986(2) \\
    $P(1 | 1)$ & 0.967(3) & 0.949(4) & 0.969(4) & 0.982(2) & 0.912(6) & 0.872(3) & 0.982(3) & 0.989(3) \\
    \hline
    \hline
\end{tabular}}
\caption{Individual readout fidelities for all qubits with excited state promotion. $P(1 | 1)$ has improved for all qubits compared to when ESP is not used. For some qubits, $P(1 | 1) > P(0 | 0)$.}
\label{tab:isolated_readout_fidelities_esp}

\bigskip

\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{l | r r r r r r r r }
    \hline
    \hline
    {} & Q0 & Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 \\
    \hline
    $P(0 | 0)$ & 0.998(2) & 0.984(4) & 0.968(3) & 0.971(3) & 0.973(2) & 0.968(3) & 0.974(4) & 0.983(3) \\
    $P(1 | 1)$ & 0.883(7) & 0.838(7) & 0.82(4) & 0.879(3) & 0.913(6) & 0.855(9) & 0.901(6) & 0.886(5) \\
    \hline
    \hline
\end{tabular}}
\caption{Simultaneous readout fidelities for all qubits without excited state promotion. We observe that readout crosstalk can improve the readout fidelity of some qubits compared to the values in Table \ref{tab:isolated_readout_fidelities}.}
\label{tab:simultaneous_readout_fidelities}

\bigskip

\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{l | r r r r r r r r }
    \hline
    \hline
    {} & Q0 & Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 \\
    \hline
    $P(0 | 0)$ & 0.989(2) & 0.976(2) & 0.965(4) & 0.964(5) & 0.967(4) & 0.956(3) & 0.975(3) & 0.985(2) \\
    $P(1 | 1)$ & 0.973(8) & 0.940(8) & 0.968(3) & 0.975(1) & 0.947(5) & 0.927(6) & 0.983(3) & 0.973(2) \\
    \hline
    \hline
\end{tabular}}
\caption{Simultaneous readout fidelities for all qubits with excited state promotion. $P(1 | 1)$ has improved for all qubits compared to when ESP is not used. For some qubits, $P(1 | 1) > P(0 | 0)$.}
\label{tab:simultaneous_readout_fidelities_esp}

\end{table*}

